Certified Training: Small Boxes are All You Need

To obtain, deterministic guarantees of adversarial robustness, specialized training methods are used. We propose, SABR, a novel such certified training method, based on the key insight that propagating interval bounds for a small but carefully selected subset of the adversarial input region is sufficient to approximate the worst-case loss over the whole region while significantly reducing approximation errors. We show in an extensive empirical evaluation that SABR outperforms existing certified defenses in terms of both standard and certifiable accuracies across perturbation magnitudes and datasets, pointing to a new class of certified training methods promising to alleviate the robustness-accuracy trade-off.

==> test-section.tex <==
\section{Test Section} \label{sec:test}

Interesting stuff:

\begin{itemize}
	\item Citations are set up already: Turing~\cite{turing1937computable}
	\item You may use UTF-8 characters: ä
	\item Use cref for references: \cref{sec:test}
	\item Reference the appendix: \cref{fig:appendix} in \cref{app:test-appendix}
	\item Use the \texttt{acro} package for acronyms: First usage: \ac{cli}, subsequent usages: \ac{cli}
\end{itemize}

\begin{figure}[t]
	\centering
	\includegraphics[height=2cm]{example-image-a}
	\caption{An example figure caption.}
	\label{fig:example}
\end{figure}

\paragraph{Figures}
See \cref{fig:example} for an example figure.

\lstinputlisting[float=t,caption={Example code.},label=lst:code]{code/example-code.psi}

\paragraph{Listings}
See \cref{lst:code} for an example Listing.

